A Dirichlet Process Mixture Model of Discrete Choice

We present a mixed multinomial logit (MNL) model, which leverages the truncated stick-breaking process representation of the Dirichlet process as a flexible nonparametric mixing distribution. The proposed model is a Dirichlet process mixture model and accommodates discrete representations of heterogeneity, like a latent class MNL model. Yet, unlike a latent class MNL model, the proposed discrete choice model does not require the analyst to fix the number of mixture components prior to estimation, as the complexity of the discrete mixing distribution is inferred from the evidence. For posterior inference in the proposed Dirichlet process mixture model of discrete choice, we derive an expectation maximisation algorithm. In a simulation study, we demonstrate that the proposed model framework can flexibly capture differently-shaped taste parameter distributions. Furthermore, we empirically validate the model framework in a case study on motorists' route choice preferences and find that the proposed Dirichlet process mixture model of discrete choice outperforms a latent class MNL model and mixed MNL models with common parametric mixing distributions in terms of both in-sample fit and out-of-sample predictive ability. Compared to extant modelling approaches, the proposed discrete choice model substantially abbreviates specification searches, as it relies on less restrictive parametric assumptions and does not require the analyst to specify the complexity of the discrete mixing distribution prior to estimation.

==> table_caseStudy_componentShares.tex <==

\centering
\begin{tabular}{@{}l 
S[table-format=2.1] S[table-format=2.1] S[table-format=2.1]
S[table-format=2.1] S[table-format=2.1] 
S[table-format=2.1] S[table-format=2.1] l@{}}

\toprule
 & \multicolumn{7}{c}{\textbf{Component number}}  \\ 
\cmidrule{2-9} 
\textbf{Model} & 
\multicolumn{1}{c}{\textbf{1}} & \multicolumn{1}{c}{\textbf{2}} & \multicolumn{1}{c}{\textbf{3}} &
\multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{\textbf{5}} & \multicolumn{1}{c}{\textbf{6}} & \multicolumn{1}{c}{\textbf{7}} & \phantom{i} \\
\midrule
LC-MNL & 29.4\% & 25.5\% & 25.0\% &  20.1\% \\

DPM-MNL & 56.2\% & 16.0\% & 3.9\% & 3.1\% & 2.9\% & 2.4\% &2.3 \%\\

\bottomrule
\end{tabular}

==> table_caseStudy_data.tex <==

\centering
\begin{tabular}{@{}p{5cm} S[table-format=1.1] S[table-format=2.1] S[table-format=2.1] S[table-format=3.1] S[table-format=2.1] S[table-format=4.0]@{}}
\toprule
\textbf{Attribute}  & \multicolumn{1}{c}{\textbf{Min.}} & \multicolumn{1}{c}{\textbf{Median}} & \multicolumn{1}{c}{\textbf{Mean}} & \multicolumn{1}{c}{\textbf{Max.}}  & \multicolumn{1}{c}{\textbf{Std. dev.}} & \multicolumn{1}{c}{\textbf{N}} \\
\midrule
\textbf{Walking} \\
\quad Walking time [minutes] &	1 & 13 & 22.8 & 150 & 31.0 & 167\\

\textbf{Bicyling} \\
\quad Bicycling time [minutes] & 1 & 21 & 23.4 & 62 & 12.0 & 460\\

\textbf{Public transportation} \\
\quad Walking time [minutes] &	2 & 3 & 4.1 & 11 & 1.7 & 382\\
\quad In-vehicle time [minutes] & 2 & 16 & 17.1 & 54 & 9.5 & 382\\
\quad Waiting time [minutes] &	2 & 4 & 4.1 & 11 & 1.7 & 382\\
\quad Number of transfers &	0 & 2 & 2.1 & 4 & 0.9 & 382\\
\quad Headway [minutes] &	5 & 20 & 33.8 & 120 & 31.5 & 382\\
\quad Share of trips with significant delays [\%] &	5 & 10 & 10.3 & 20 & 5.9 & 382\\
\quad Travel cost [EUR] &	0.1 & 1.8 & 1.8 & 3.2 & 0.5 & 382\\

\textbf{Car} \\
\quad Walking time [minutes] &	2 & 3 & 3.6 & 11 & 1.4 & 1441\\
\quad Time spent driving [minutes] & 2 & 12 & 12.8 & 52 & 7.7 & 1441\\
\quad Time spent in congested conditions [minutes] & 0 & 2 & 2.3 & 11 & 1.6 & 1441\\
\quad Share of trips with significant delays [\%] &	5 & 10 & 11.1 & 20 & 6.2 & 1441\\
\quad Travel cost [EUR] &	0.2 & 1.6 & 1.6 & 3.6 & 0.7 & 1441\\
\bottomrule
\end{tabular}

==> table_caseStudy_res1.tex <==

\centering
\begin{tabular}{@{}l S[table-format=1.3] S[table-format=1.3] c S[table-format=1.3] S[table-format=1.3] @{}}
\toprule
 & \multicolumn{2}{c}{\textbf{MNL}} & \phantom{a} & \multicolumn{2}{c}{\textbf{M-MNL}}  \\
\cmidrule{2-3} \cmidrule{5-6} 
\textbf{Coefficient} & \multicolumn{1}{c}{\textbf{Est.}}  & \multicolumn{1}{c}{\textbf{Std. err.}} & & \multicolumn{1}{c}{\textbf{Est.}}  & \multicolumn{1}{c}{\textbf{Std. err.}} \\
\midrule
Alternative-specific constants \\
\quad Car \\
\quad \quad Location & 0.000$^{\#}$ & && 0.000$^{\#}$ & \\
\quad \quad Scale & & && -1.504$^{***}$ & 0.187 \\
\quad Walking \\
\quad \quad Location & -0.866$^{***}$ & 0.057 && 1.189$^{***}$ & 0.144 \\
\quad \quad Scale & & && -1.253$^{***}$ & 0.213 \\
\quad Bicycling \\
\quad \quad Location& -4.076$^{***}$ & 0.084 && -7.173$^{***}$ & 0.575 \\
\quad \quad Scale & & && 3.230$^{***}$ & 0.349 \\
\quad Public transit \\
\quad \quad Location & -0.907$^{***}$ & 0.072 && 1.472$^{***}$ & 0.195 \\
\quad \quad Scale & & && -0.636$^{***}$ & 0.476 \\

Travel cost [USD] & -0.206$^{***}$ & 0.014 && -0.087$^{***}$ & 0.008 \\

In-vehicle time [hours]  \\
\quad Location & -0.709$^{***}$ & 0.068 && -1.013$^{***}$ & 0.085 \\
\quad Scale & & && 0.895$^{***}$ & 0.010 \\

Out-of vehicle time [hours] \\
\quad Location & -0.755$^{***}$ & 0.025 && -3.649$^{***}$ & 0.137\\
\quad Scale & & &&   1.744$^{***}$ & 0.075 \\

\midrule
\multicolumn{6}{l}{$^{***}$ p-value $<0.01$; $^{**}$ p-value $<0.05$; $^{*}$ p-value $<0.10$}\\
\multicolumn{6}{l}{$^{\#}$ fixed for identification}\\
\bottomrule
\end{tabular}

==> table_caseStudy_res2.tex <==

\centering
\begin{tabular}{@{}l S[table-format=1.3] S[table-format=1.3] c S[table-format=2.3] S[table-format=1.3] @{}}
\toprule
 & \multicolumn{2}{c}{\textbf{LC-MNL}} & \phantom{a} & \multicolumn{2}{c}{\textbf{DPM-MNL}}  \\
\cmidrule{2-3} \cmidrule{5-6} 
\textbf{Coefficient} & \multicolumn{1}{c}{\textbf{Est.}}  & \multicolumn{1}{c}{\textbf{Std. err.}} & & \multicolumn{1}{c}{\textbf{Est.}}  & \multicolumn{1}{c}{\textbf{Std. err.}} \\
\midrule
\textbf{Generic coefficients}\\
\quad Travel cost [USD] & -0.087$^{***}$ & 0.008 && -0.083$^{***}$ & 0.008 \\
\midrule

\textbf{Component 1} & \multicolumn{2}{l}{\textbf{Share: 65.0\%}} && \multicolumn{2}{l}{\textbf{Share: 85.6\%}} \\
\quad Alternative-specific constants \\
\quad \quad Walking & 2.149$^{***}$ & 0.109 && 1.685$^{***}$ & 0.088 \\
\quad \quad Bicycling & -2.308$^{***}$ & 0.112 && -3.232$^{***}$ & 0.102 \\
\quad \quad Public transit & 1.620$^{***}$ & 0.114 && 1.332$^{***}$ & 0.107 \\
\quad In-vehicle time [hours]  & -0.569$^{**}$ & 0.251 && -0.983$^{***}$ & 0.020 \\
\quad Out-of vehicle time [hours] & -4.976$^{***}$ & 0.305 && -2.979$^{***}$ & 0.101\\
\midrule

\textbf{Component 2} & \multicolumn{2}{l}{\textbf{Share: 30.2\%}} && \multicolumn{2}{l}{\textbf{Share: 8.6\%}} \\
\quad Alternative-specific constants \\
\quad \quad Walking & 2.149$^{***}$ & 0.109 && 1.685$^{***}$ & 0.088 \\
\quad \quad Bicycling & -2.308$^{***}$ & 0.112 && -3.232$^{***}$ & 0.102 \\
\quad \quad Public transit & 1.620$^{***}$ & 0.114 && 1.332$^{***}$ & 0.107 \\
\quad In-vehicle time [hours]  & -1.376$^{***}$ & 0.152 && -1.746$^{***}$ & 0.321 \\
\quad Out-of vehicle time [hours] & -1.785$^{***}$ & 0.077 && -1.083$^{***}$ & 0.218\\
\midrule

\textbf{Component 3} & \multicolumn{2}{l}{\textbf{Share: 4.8\%}} && \multicolumn{2}{l}{\textbf{Share: 3.2\%}} \\
\quad Alternative-specific constants \\
\quad \quad Walking & 2.149$^{***}$ & 0.109 && 1.685$^{***}$ & 0.088 \\
\quad \quad Bicycling & -2.308$^{***}$ & 0.112 && -3.232$^{***}$ & 0.102 \\
\quad \quad Public transit & 1.620$^{***}$ & 0.114 && 1.332$^{***}$ & 0.107 \\
\quad In-vehicle time [hours]  & -0.398$^{***}$ & 0.105 && -0.287$^{***}$ & 0.068 \\
\quad Out-of vehicle time [hours] & -0.060$^{**}$ & 0.023 && 0.010 & 0.055\\
\midrule

\textbf{Component 4} & & && \multicolumn{2}{l}{\textbf{Share: 1.7\%}} \\
\quad Alternative-specific constants \\
\quad \quad Walking & 2.149$^{***}$ & 0.109 && 1.685$^{***}$ & 0.088 \\
\quad \quad Bicycling & -2.308$^{***}$ & 0.112 && -3.232$^{***}$ & 0.102 \\
\quad \quad Public transit & 1.620$^{***}$ & 0.114 && 1.332$^{***}$ & 0.107 \\
\quad In-vehicle time [hours]  &  & && -34.754$^{***}$ & 0.259 \\
\quad Out-of vehicle time [hours] & & && -40.280$^{***}$ & 0.718\\
\midrule

\textbf{Component 5} & & && \multicolumn{2}{l}{\textbf{Share: 1.7\%}} \\
\quad Alternative-specific constants \\
\quad \quad Walking & 2.149$^{***}$ & 0.109 && 1.685$^{***}$ & 0.088 \\
\quad \quad Bicycling & -2.308$^{***}$ & 0.112 && -3.232$^{***}$ & 0.102 \\
\quad \quad Public transit & 1.620$^{***}$ & 0.114 && 1.332$^{***}$ & 0.107 \\
\quad In-vehicle time [hours]  &  & && -34.754$^{***}$ & 0.259 \\
\quad Out-of vehicle time [hours] & & && -40.280$^{***}$ & 0.718\\
\midrule

\multicolumn{6}{l}{$^{***}$ p-value $<0.01$; $^{**}$ p-value $<0.05$; $^{*}$ p-value $<0.10$}\\
\bottomrule
\end{tabular}

==> table_sensitivityAnalysis.tex <==

\centering
\begin{tabular}{@{}l 
S[table-format=4.1] S[table-format=4.1] S[table-format=4.1] @{}}

\toprule
 & \multicolumn{3}{c}{\textbf{Truncation level, upper limit on}}  \\ 
\cmidrule{2-4} 
$G_{0}$ & 
\multicolumn{1}{c}{$K = 50$, $\alpha_{U} = 10$} & \multicolumn{1}{c}{$K = 100$, $\alpha_{U} = 20$} & \multicolumn{1}{c}{$K = 150$, $\alpha_{U} = 30$} \\
\midrule
$\mbox{N}(0,1^{2})$   -2610.0  & -2669.5 & -2647.0 \\
$\mbox{N}(0,10^{2})$     & -2599.1 & -2574.8 & 0 \\
$\mbox{N}(0,100^{2})$  & -2583.4 & -2565.1 & -2.6429 \\
\bottomrule
\end{tabular}

==> table_simStudy_fit.tex <==

\centering
\begin{tabular}{@{}l 
S[table-format=4.1] S[table-format=4.1] S[table-format=4.1] S[table-format=4.1] @{}}

\toprule
 & \multicolumn{4}{c}{\textbf{Experiment}}  \\ 
\cmidrule{2-5} 
\textbf{Model} & 
\multicolumn{1}{c}{\textbf{I}} & \multicolumn{1}{c}{\textbf{II}} & \multicolumn{1}{c}{\textbf{III}} &
\multicolumn{1}{c}{\textbf{IV}} \\
\midrule
MNL          & -3230.7 & -8724.1 & -3578.4 & -3437.3\\
M-MNL      & -2655.4 & -4481.3 & -3137.3 & -2972.0\\
DPM-MNL & -2695.9 & -4822.7 & -3049.9 & -2948.2\\
\bottomrule
\end{tabular}

==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}
